SeaExam and SeaBench: Benchmarking LLMs with Local Multilingual Questions in Southeast Asia

This study introduces two novel benchmarks, SeaExam and SeaBench, designed to evaluate the capabilities of Large Language Models (LLMs) in Southeast Asian (SEA) application scenarios. Unlike existing multilingual datasets primarily derived from English translations, these benchmarks are constructed based on real-world scenarios from SEA regions. SeaExam draws from regional educational exams to form a comprehensive dataset that encompasses subjects such as local history and literature. In contrast, SeaBench is crafted around multi-turn, open-ended tasks that reflect daily interactions within SEA communities. Our evaluations demonstrate that SeaExam and SeaBench more effectively discern LLM performance on SEA language tasks compared to their translated benchmarks. This highlights the importance of using real-world queries to assess the multilingual capabilities of LLMs.

==> latex/tables/corr_by_cate_SeaBench.tex <==
\begin{table}[h!]
\centering
\small
    \begin{tabular}{lcccc}
        \toprule
        category & \textbf{id} & \textbf{th} & \textbf{vi} & \textbf{avg} \\ 
        \midrule
        math & 0.98 & 0.97 & 0.82 & 0.92 \\ 
        coding & 0.82 & 0.91 & 0.87 & 0.87 \\ 
        stem & 0.76 & 0.91 & 0.80 & 0.82 \\ 
        writing & 0.92 & 0.85 & 0.70 & 0.82 \\ 
        extraction & 0.88 & 0.82 & 0.72 & 0.81 \\ 
        humanities & 0.61 & 0.96 & 0.68 & 0.75 \\ 
        roleplay & 0.63 & 0.82 & 0.68 & 0.71 \\ 
        reasoning & 0.62 & 0.97 & 0.44 & 0.68 \\ 
        \bottomrule
    \end{tabular}
\caption{The ranking correlation between SeaBench and MT-bench-SEA for each language and category.}
\label{tab:corr_seabench_cate}
\end{table}

==> latex/tables/corr_by_lang_SeaBench.tex <==
\begin{table}[h!]
\centering
\setlength\tabcolsep{4.5pt}
\small
\begin{tabular}{lcccc}
\toprule
 & \textbf{id} & \textbf{th} & \textbf{vi} & \textbf{avg} \\
\midrule
Corr(SeaBench, MT-SEA) & 0.95 & 0.95 & 0.90 & 0.93 \\
Corr(SeaBench, MT-human) & 0.92 & 0.92 & 0.92 & 0.92 \\
Corr(MT-SEA, MT-human) & \textbf{0.98} & \textbf{0.98} & \textbf{0.97} & \textbf{0.98} \\

\bottomrule
\end{tabular}
\caption{The ranking correlation between SeaBench and translated MT-bench for each language. "MT-SEA" is short for "MT-bench-SEA", and "MT-human" is short for "MT-bench-SEA-human"}
\label{tab:corr_seabench_lang}
\end{table}



==> latex/tables/corr_by_lang_SeaExam.tex <==


\begin{table}[h!]
\centering
\small
\begin{tabular}{lcccc}
\toprule
 & \textbf{id} & \textbf{th} & \textbf{vi} & \textbf{avg} \\
\midrule
% \textbf{Corr} & 0.93 & 0.98 & 0.97 & 1.0 \\
% \textbf{Corr} & 0.88 & 0.97 & 0.97 & 1.0 \\
\textbf{Corr} & 0.88 & 0.97 & 0.97 & 0.94 \\
\bottomrule
\end{tabular}
\caption{The ranking correlation between SeaExam and MMLU-SEA for each language. ‘avg' means the average ranking correlations across the three languages.}
\label{tab:corr_seaExam}
\end{table}

==> latex/tables/mt-bench-example.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{p{0.1\textwidth}p{0.85\textwidth}}
    \toprule
        language &  instruction \\
        \midrule
        en & \textbf{Turn 1}: Compose an engaging travel blog post about a recent trip to Hawaii, highlighting cultural experiences and must-see attractions. \newline
        \textbf{Turn 2}: Rewrite your previous response. Start every sentence with the letter A. \\

        \midrule
        id & \textbf{Turn 1}: Tulis postingan blog perjalanan yang menarik tentang perjalanan baru-baru ini ke Hawaii, yang menyoroti pengalaman budaya dan atraksi yang wajib dikunjungi. \newline 
        \textbf{Turn 2}: Tulis ulang tanggapan Anda sebelumnya. Mulailah setiap kalimat dengan huruf A.\\
        \midrule 
        vi & \textbf{Turn 1}: Soạn một bài đăng blog du lịch hấp dẫn về chuyến đi gần đây đến Hawaii, nêu bật những trải nghiệm văn hóa và những điểm tham quan không thể bỏ qua.\newline 
        \textbf{Turn 2}: Viết lại phản hồi trước đó của bạn. Bắt đầu mỗi câu bằng chữ A.\\
        \midrule
        th & \textbf{Turn 1}: เขียนโพสต์บล็อกการเดินทางที่น่าสนใจเกี่ยวกับการเดินทางไปฮาวายครั้งล่าสุด โดยเน้นประสบการณ์ทางวัฒนธรรมและสถานที่ท่องเที่ยวที่ต้องไปชม\newline 
        \textbf{Turn 2}: เขียนคำตอบก่อนหน้าของคุณใหม่ เริ่มต้นทุกประโยคด้วยตัวอักษร A\\
    \bottomrule
    \end{tabular}
    \caption{SeaBench translation example.}
    \label{tab:mt-bench_example}
\end{table*}

==> latex/tables/seaBench_type_correlation.tex <==
\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{lc}
    \toprule
        \textbf{Category} & \textbf{Spearman correlation (\%)} \\ 
        \midrule
        coding & 95.0 \\ 
        math & 93.3 \\ 
        STEM & 91.7 \\ 
        humanities & 87.0 \\ 
        reasoning & 86.7 \\ 
        roleplay & 85.0 \\ 
        extraction & 76.2 \\ 
        writing & 73.3 \\ 
    \bottomrule
    \end{tabular}
    \caption{Spearman's rank correlation for each category between SeaBench and MT-bench-SEA.}
    \label{tab:corr_seaBench_type}
\end{table}

==> latex/tables/stats_mt_bench_seabench.tex <==
\begin{table*}[h!]
\centering
\small
\setlength\tabcolsep{4pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{p{0.1\textwidth}p{0.6\textwidth}p{0.1\textwidth}p{0.12\textwidth}}
\toprule
\textbf{Dataset} & \textbf{Categories} & \textbf{Languages} & \textbf{\# Samples} \\ 
\midrule
MT-bench & Writing, Math, Reasoning, STEM, Roleplay, Extraction, Humanities, Coding & en & 80 \\ 
SeaBench & Writing, Math, Reasoning, STEM, Roleplay, Extraction, Humanities, Coding, \textbf{Safety}, \textbf{Life} & id, th, vi & 300 \\ 
\bottomrule
\end{tabular}
}
\caption{Comparison of MT-bench and SeaBench. The additional categories in SeaBencha are in \textbf{bold}.}
\label{tab:stats_mt_seabench}
\end{table*}
